On the interplay between data structure and loss function in classification problems

One of the central puzzles in modern machine learning is the ability of heavily overparametrized models to generalize well. Although the low-dimensional structure of typical datasets is key to this behavior, most theoretical studies of overparametrization focus on isotropic inputs. In this work, we instead consider an analytically tractable model of structured data, where the input covariance is built from independent blocks allowing us to tune the saliency of low-dimensional structures and their alignment with respect to the target function. Using methods from statistical physics, we derive a precise asymptotic expression for the train and test error achieved by random feature models trained to classify such data, which is valid for any convex loss function. We study in detail how the data structure affects the double descent curve, and show that in the over-parametrized regime, its impact is greater for logistic loss than for mean-squared loss: the easier the task, the wider the gap in performance at the advantage of the logistic loss. Our insights are confirmed by numerical experiments on MNIST and CIFAR10.

==> checklist.tex <==
\clearpage
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{The main limitation of our work is the informal statement of our analytical results, which are based on non-rigorous tools from Statistical Physics. Making our claims fully rigorous is outside the scope of this paper but can likely be done by exploiting recent results in the litterature: we provide a thorough discussion of this in the introduction.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{This is a purely theoretical contribution.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{We provide a detailed derivation of all theoretical results in SM.~\ref{app:replica}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Provided in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In the captions of the figures.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Numerical results are all averaged over 10 runs, and come with error bars.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{Experiments all run on a laptop.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> dfdxcbxrhpmwxgqmtdsvvrxqthrzkvjb/abstract.tex <==

\begin{abstract}

One of the central features of deep learning is the generalization abilities of neural networks, which seem to improve relentlessly with over-parametrization.
In this work, we investigate how properties of data impact the test error as a function of the number of training examples and number of training parameters; in other words, how the structure of data shapes the ``generalization phase space".
We first focus on the random features model trained in the teacher-student scenario. The synthetic input data is composed of independent blocks, which allow us to tune the saliency of low-dimensional structures and their relevance with respect to the target function.
Using methods from statistical physics, we obtain an analytical expression for the train and test errors for both regression and classification tasks in the high-dimensional limit. The derivation allows us to show that noise in the labels and strong anisotropy of the input data play similar roles on the test error. 
Both promote an asymmetry of the phase space where increasing the number of training examples improves generalization further than increasing the number of training parameters.
Our analytical insights are confirmed by numerical experiments involving fully-connected networks trained on MNIST and CIFAR10.
\end{abstract}


% One of the central features of deep learning is the generalization abilities of neural networks, which seem to improve relentlessly with over-parametrization. In practice, the ability to generalize depends both on the number of parameters,  $P$, and the number of samples used to train the network, $N$. In this work, we investigate  ``generalization phase-space", i.e. the test error dependence on $N$ and $P$. 

% what are the main properties of the data that determine the

% We first focus on a  model of random features, trained on synthetic data 
% in which we can tune the relevance of low-dimensional structures and their saliency with respect to the the target function.
% By using methods from statistical physics, we obtain an analytical expression for the train and test errors for both regression and classification tasks in the high-dimensional limit. This allows us to show that noise in the labels and strong 
% anisotropy of the input data play a similar role. Both promote an asymmetry of the phase-space where increasing sample size $N$ improves generalization further than increasing fitting model size $P$.
% We also provide a detailed analysis of the role of the data structure on the double descent curve. Our analytical results are confirmed by numerical experiments on neural networks trained on realistic data sets, in which we vary the strength of the label noise by corrupting labels and we vary the anisotropy by applying a PCA transformation. 




% v1
%In this work, we investigate the generalization phase space starting from the following observation: On \textit{simple} datasets, a fully-connected network with $P$ parameters trained on $N$ samples typically reaches the same performance as the network with $N$ parameters trained on $P$ samples. Then we explore when this symmetry holds or breaks depending on the structure of data and noise in the labels. More precisely, we empirically show that when the labels are corrupted or when the inputs are replaced by their principal components, the generalization phase space symmetry is broken in favor of having more data over having more parameters.
%To understand this phenomenon, we consider an analytically tractable model of random features, trained on a synthetic data with an adjustable structure.
%Using methods from statistical physics, we obtain a precise expression for the train and test error for both regression and classification tasks 
%in the high-dimensional limit.
%We provide a detailed analysis of the effect of data structure on the double descent curve and recover the $N\text{-}P$ symmetry breaking when the data becomes anisotropic, or the labels are corrupted.


%v0
% One of the main puzzles in deep learning is the generalization abilities of neural networks, which seem to improve relentlessly with overparametrization. 
% In this work, we start from the surprising observation that a fully-connected network with $P$ parameters trained on $N$ examples 
% on simple datasets from MNIST or CIFAR10 
% reaches almost exactly the same performance as one with $N$ parameters trained on $P$ examples. 
% This curious symmetry is nonetheless broken when the labels are corrupted or when the inputs are replaced by their principal components
% : the resulting noise gives an 
% advantage to having more data over having more parameters.
% To gain deeper understanding on this phenomenology, we consider an analytical tractable model of random features, trained on a structured anisotropic dataset. We obtain a precise expression for the train and test error for both regression and classification tasks, and reveal a particularly simple relation between train and test loss for regression. We provide a detailed analysis of the effect of data structure on the double descent curve, and recover the $N,P$ symmetry breaking when the data becomes anisotropic or the labels are corrupted.

==> dfdxcbxrhpmwxgqmtdsvvrxqthrzkvjb/acknowledgements.tex <==
\paragraph{Acknowledgements}
We thank Berfin Simsek, Armand Joulin, Bruno Loureiro, Federica Gerace for helpful discussions. SD and GB acknowledge funding from the French government under management of Agence Nationale de la Recherche as part of the “Investissements d’avenir” program, reference ANR-19-P3IA-0001 (PRAIRIE 3IA Institute). MG acknowledges funding from the Flatiron Institute. We also thank Lenka Zdeborova and Florent Krzakala, and Les Houches Summer School for organizing a workshop on
Statistical Physics and Machine Learning where this work was partially done. 

==> dfdxcbxrhpmwxgqmtdsvvrxqthrzkvjb/deprecated/introduction.tex <==
Most analytical studies of generalization in machine learning consider the simplistic setup where the input data is taken to be i.i.d., sampled from a standard gaussian of unit variance. Although this scenario enables the understand of many phenomena such as the overfitting peaks which occur near interpolation thresholds, it is far from the being sufficient to understanding the phenomenology observed on real-world datasets such as MNIST.

Of prime importance to understand the role of structure in data is the covariance structure of the input data. Real-world datasets are strongly correlated, and most of their information is carried in their first principal components. 

In this work, we consider random feature regression as a proxy for lazy learning. We consider the high-dimensional setup where the number of training examples $N$, the number of parameters $P$ and the input dimension $D$ are all sent to infinity with their ratios fixed. 

\subsection{General setup}

\paragraph{Dataset} The input data $\bs X\in\sR^{N\times D}$ consists of $N$ vectors in $D$ dimensions whose elements are drawn i.i.d. from $\mathcal{N}(0,\bs \Sigma)$. For each model, there is an associated label generator $f^\star$ corrupted by additive Gaussian noise: $y=f^\star(\bs x) + \epsilon$, where the noise variance is inversely related to the signal to noise ratio (SNR), $\epsilon \sim \mathcal {N}(0, 1/\mathrm{SNR})$. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/RF.pdf}
  \caption{Illustration of an RF network. }
  \label{fig:rf}
\end{figure}

\paragraph{Model} 
We consider the random features (RF) model introduced in \cite{rahimi2008random}. It can be viewed as a two-layer neural network whose first layer is a fixed random matrix $\bs \Theta\in \sR^{P \times D}$ (see Fig.~\ref{fig:rf})\footnote{This model, shown to undergo double descent in~\cite{mei2019generalization}, has become a cornerstone to study the so-called lazy learning regime of neural networks where the weights stay close to their initial value~\cite{jacot2018neural}: assuming $f_{\theta_0}\!=\!0$, we have $f_{\theta}({\bf x}) \approx \nabla_{\theta}f_{\theta}({\bf x})|_{\theta\!=\!\theta_0} \cdot (\theta-\theta_0)$~\cite{chizat2018note}. In other words, lazy learning amounts to a linear fitting problem with a random feature vector $\left.\nabla_{\theta}f_{\theta}({\bf x})\right|_{\theta\!=\!\theta_0}$.}:
    \begin{equation}
        f(\vx)=\sum_{i=1}^P\va_i \sigma\left(\frac{\langle\bs \Theta_i, \vx\rangle}{\sqrt{D}}\right).
\end{equation} 
$\sigma$ is a pointwise activation function, the choice of which will be of prime importance in the study. The ground truth is a linear model given by $f^\star(\bs x)=\langle\bs \beta,\bs x \rangle / \sqrt D$. Elements of $\bs \Theta$ and $\bs \beta$ are drawn i.i.d from $\mathcal{N}(0,1)$.

\paragraph{Training} The second layer weights, i.e. the elements of $\va$, are calculated via ridge regression with a regularization parameter $\gamma$:
\begin{align}
    \boldsymbol{\hat a} &=  \underset{\boldsymbol{a} \in \sR^{P}}{\arg \min }\left[ \frac{1}{N}\left(\bs y-\va \bf Z^\top \right)^{2}+\frac{P \gamma}{D}\|\boldsymbol{a}\|_{2}^{2}\right] = \frac{1}{N}\bs y^\top \bs Z \left( \bs \Sigma + \frac{P\gamma}{D} \mathbb{I}_P\right)^{-1} \\
    \bs Z_i^\mu &= \sigma\left(\frac{\langle\bs \Theta_i, \bs X_\mu\rangle}{\sqrt{D}}\right) \in \sR^{N\times P}, \quad \bs \Sigma = \frac{1}{N}\bs Z^\top \bs Z \in \sR^{P\times P}
\label{eq:estimator}
\end{align}

\subsection{Covariance structure}

To study the impact of the structure of the dataset, we consider two models for the covariance matrix $\bs \Sigma$: 
\begin{itemize}
    \item \textbf{Spiked tensor model}: the covariance matrix presents one large eigenvalue popping out of the bulk: $\bs \Sigma = \mathbb I_d + c \bs v \bs v^\top$. Without loss of generality, we take $\bs v = \vec 1 = (1\ 1\ ...)^\top$, hence we have $\bs \Sigma_{ij} = \delta_{ij} + c(1-\delta_{ij})$.
    \item \textbf{Strong and weak features model}: we have two eigenspaces $E_1, E_2$ of strengths $\lambda_1, \lambda_2$ and of extensive sizes $d_1 = \phi_1 d$ and $d_2 = \phi_2 d$. We denote the projected squared norm of the teacher in both eigenspaces: $\beta_i = \frac{1}{d} \Vert \bs \theta^0_i \Vert^2$.
\end{itemize}

The spiked tensor model is a classic model in the statistics litterature, but the special direction $\vec 1$ is usually used as the teacher vector which the learner must find despite the ambient noise~\cite{baik2005phase}. Here, the special direction is simply used to break the anisotropy, but it is by no means the true signal.

The strong and weak features model has been recently studied empirically~\cite{nakkiran2020optimal} and theoretically~\cite{wu2020optimal,richards2020asymptotics} in the context of least-squares regression. In this model, it was shown that the two subspaces gives rise to two peaks instead of one in the double descent curve. 

An intriguing observation which emerges in strongly anisotropic data is that the optimal ridge regularization parameter $\gamma$ can actually become negative~\cite{wu2020optimal,kobak2019optimal}. Indeed, if a few directions carry the most variance, trying to decrease the $\ell_2$ norm of the weights is detrimental: on the contrary, one would want to encourage a few directions to become strong and the rest to become zero, as is encouraged by $\ell_1$ regularizaton or $\ell_2$ with a negative ridge.



==> dfdxcbxrhpmwxgqmtdsvvrxqthrzkvjb/deprecated/main_text_old.tex <==
\section{Introduction}

A few years ago, deep neural networks achieved breakthroughs in a variety of contexts~\cite{krizhevsky2012imagenet, lecun2015deep,hinton2012deep,sutskever2014sequence}. However, their remarkable generalization abilities have puzzled rigorous understanding~\cite{zhang2016understanding,advani2017high,neyshabur2018towards}: classical learning theory predicts that generalization error should follow a U-shaped curve as the number of parameters $P$ increases, and a monotonous decrease as the number of training examples $N$ increases. Instead, recent developments show that deep neural networks, as well as other machine learning models, exhibit a starkly different behaviour. In the absence of regularization, increasing $P$ and $N$ respectively yields parameter-wise and sample-wise \emph{double descent} curves~\cite{belkin2018reconciling,geiger2020scaling,spigler2019jamming,mei2019generalization, nakkiran2019deep,nakkiran2019more}, whereby the generalization error first decreases, then peaks at the \emph{interpolation threshold} (at which point training error vanishes), then decreases monotonically again. This peak\footnote{Also called the \emph{jamming} peak due to similarities with a well-studied phenomenon in the Statistical Physics literature~\cite{opper1996statistical,engel2001statistical,krzakala2007landscape,franz2016simplest,geiger2019jamming}.} was shown to be related to a sharp increase in the variance of the estimator \cite{geiger2019jamming,geiger2020scaling,d2020double}.
%Of prime importance is therefore to understand why increasing the number of parameters in a learning model seems to play a similar role to increasing the number of examples in the dataset. 

However, the phenomenology mentioned above was mainly derived in the simplistic setup of square loss regression, where the input data is taken to be i.i.d., sampled from a standard Gaussian of unit variance. Although this scenario enables the understanding of many phenomena such as the overfitting peaks which occur near interpolation thresholds, it is far from being sufficient to understanding the phenomenology observed in deep learning, that of classification tasks on real-world datasets. 

\subsection{Approach}

\paragraph{Strong and weak features model}

To mimick a structured dataset, we start from the observation that real-world datasets are strongly correlated, and most of their information is carried in their first principal components. To mimick this effect in the simplest possible way, we introduce a block model in which the elements of the inputs $\bs x\in \mathbb R^D$ and the teacher $\bs \beta \in \sR^D$ are sampled from a centered Gaussian distribution whose covariance has the following block structure:
\begin{align*}
&\bs x\sim\mathcal{N}(0, \Sigma_x),  &&\Sigma_x = \begin{bmatrix}
\sigx{1} \mathbb I_{\phi_1 D} & 0 & 0\\
0 & \sigx{2} \mathbb I_{\phi_2 D} & 0\\
0 & 0 & \ddots
\end{bmatrix}\\
&\bs \beta \sim\mathcal{N}(0, \Sigma_\beta),  &&\Sigma_\beta = \begin{bmatrix}
\sigb{1} \mathbb I_{\phi_1 D} & 0 & 0 \\
0 & \sigb{2} \mathbb I_{\phi_2 D} & 0\\
0 & 0 & \ddots
\end{bmatrix}\\
\end{align*}

Although our theory is valid (at no extra burden) for an arbitrary number of blocks, we will focus special case of our setup and consider only two blocks of sizes $\phi_1,\phi_2$. We will typically be interested in the strongly anisotropic setup where the first subspace is much smaller $\phi_1 \ll 1$, but potentially has higher \emph{saliency} ($r_x = \sigx{1}/ \sigx{2} \gg 1$) or more relevance \emph{relevance} ($r_\beta = \sigb{1}/ \sigb{2} \gg 1$).

\paragraph{Contribution}

We present an analytical derivation of the train and test error of a random feature model trained on the strong and weak features model. The tasks considered include regression with additive gaussian noise and classification with random label flipping. Our derivation builds on the methods introduced in~\cite{gerace2020generalisation}, and leverages other tools from Statistical Mechanics. 

Of particular interest is examining how the structure of the strong and weak model affect the sample-wise and parameter-wise double descent curves. To this end, we broadly study the $(N,P)$ phase space of the generalization error, following the lines of~\cite{d2020triple}. We observe that in the isotropic scenario, this phase space is symmetric, indicating that having few data but many parameters is equivalent to having few parameters but many data. We observe that this curious symmetry vanishes either when noise is added to the labels, or when the data becomes anisotropic. We confirm these observations with two-layer networks trained on MNIST and CIFAR10.

\subsection{Related Work}

\paragraph{Structure of data} 
Although most theoretical studies of generalization focus on structureless data, a few exceptions exist. The strong and weak features model has recently been studied in the context of least-squares regression, both empirically~\cite{nakkiran2020optimal} and theoretically~\cite{wu2020optimal,richards2020asymptotics}. Several intriguing observation emerge in strongly anisotropic setup : (i) several overfitting peaks can be seen ~\cite{nakkiran2020optimal,chen2020multiple} ; (ii) the optimal ridge regularization parameter $\gamma$ can become negative~\cite{wu2020optimal,kobak2019optimal}, as it becomes helpful to encourage the weights to have very different norms ; (iii) extra features acting as pure noise can actually play a beneficial role by inducing some implicit regularization\cite{richards2020asymptotics}.

The strong and weak feature model also includes the setup studied in~\cite{ghorbani2020neural}, called the spiked covariates model, where the larger of the two blocks has no correlation with the labels, i.e. $\beta_2=0$. This useless part of the input is called "junk". The question is then : can RKHS methods learn to discard these junk features hence "beating the curse of dimensionality" in the way neural networks do ? The answer was shown to depend on the strength of the junk features : when $\sigx{2}$ is small, then they are not problematic and the RKHS method ignores them, effectively learning a task of dimensionality $\phi_1 D \ll D$.

More general models of data structure were considered in other works. In the special case of random Fourier Feature regression, \cite{liao2020random} derived the train and test error for a general input distribution. \cite{canatar2020statistical} achieved a similar result in the non-parametric setting of kernel regression, which can be viewed as the limiting case of random feature regression where the number of random features goes to infinity.

On a different line, \cite{ortiz2020neural} studied the inductive bias of neural networks through their Neural Anisotropy Directions (NAD), i.e. the directions in input space along which they are best at learning. They showed that although fully-connected architectures are isotropic in nature, more specific architectures have a more intricate NAD structure. \cite{li2019towards} studied the effect of "hard-to-fit, easy-to-generalize" features, which are very akin to our strong and weak feature model. They show that large learning rates favor the fitting of easy-to-fit, hard-to-generalize features (what we would call highly salient but little relevant), whereas small learning rate does the opposite, motivating the use of learning rate decay.

\paragraph{Regression versus classification}
The few works studying classification analytically have mostly focused on linear models, trained on linearly separable data~\cite{montanari2019generalization,chatterji2020finite,liang2020precise} or gaussian mixtures~\cite{deng2019model,mignacco2020role}. The major difference with respect to the regression setup is the larger freedom of loss function which can be used~\cite{kini2020analytic,muthukumar2020classification}, which in particular changes the location of the interpolation threshold. 

A notable exception is~\cite{gerace2020generalisation}, on which this paper builds. Using tools from Statistical Mechanics, the authors were able to derive the generalization loss of random features models applied to isotropic data for any loss function. 

\section{Setup and analytical results}

\paragraph{Task}
\begin{figure}
    \centering
    \includegraphics[width=.6\columnwidth]{RF.pdf}
    \includegraphics[width=.9\columnwidth]{Data.pdf}
    \caption{\textit{Left:} Random feature model considered here. \textit{Right:} Strong and weak features model considered here.}
    \label{fig:RF}
\end{figure}
We consider the random features (RF) model introduced in \cite{rahimi2008random}.\footnote{This model, shown to undergo double descent in~\cite{mei2019generalization}, has become a cornerstone to study the so-called lazy learning regime of neural networks where the weights stay close to their initial value~\cite{jacot2018neural}: assuming $f_{\theta_0}\!=\!0$, we have $f_{\theta}({\bf x}) \approx \nabla_{\theta}f_{\theta}({\bf x})|_{\theta\!=\!\theta_0} \cdot (\theta-\theta_0)$~\cite{chizat2018note}. In other words, lazy learning amounts to a linear fitting problem with a random feature vector $\left.\nabla_{\theta}f_{\theta}({\bf x})\right|_{\theta\!=\!\theta_0}$.}
%Our setup is similar to ~\cite{gerace2020generalisation}.  
It can be viewed as a two-layer neural network whose first layer has a fixed random weight matrix $\bs F\in \sR^{P \times D}$:
\begin{equation}
    \hat y^\mu = \hat f\left(\sum_{i=1}^P\bs w_i \sigma\left(\frac{\langle\bs F_i, \bs x^\mu\rangle}{\sqrt{D}}\right)\right)\equiv \hat f\left(\bs w\cdot \bs z^\mu \right).
\end{equation} 
where $\sigma(\cdot)$ is a pointwise activation function and we introduced the notation $\bs z^\mu \in \sR^P$.
Elements of $\bs F$ are drawn i.i.d from $\mathcal{N}(0,1)$.  The labels are given by a linear ground truth, modulated by an output function $f^0$ and possibly corrupted by noise through a probabilistic channel $\gP$ :
\begin{equation}
    \label{eq:teacher-def}
    y^\mu \sim \gP \left( \cdot \left\vert  f^0\left(\frac{\langle\bs \beta,\bs x^\mu \rangle}{\sqrt D}\right)\right.\right).
\end{equation}

The second layer weights, i.e. the elements of $\bs w \in \sR^P$, are trained by minimizing 
% using 
a $\ell_2$-regularized loss on $N$ samples:
\begin{align}
    \hat{\boldsymbol{w}}=\underset{\boldsymbol{w}}{\operatorname{argmin}}\left[\sum_{\mu=1}^{N} \ell\left(y^{\mu}, \bs w \cdot \bs z^\mu \right)+\frac{\lambda}{2}\|\boldsymbol{w}\|_{2}^{2}\right].
\end{align}
We consider both regression tasks, where $\hat f = f^0 = \text{id}$, and binary classification tasks, $\hat f = f^0 = \text{sign}$. In the first case, $\ell$ is the square loss and the noise is additive. In the second case, $\ell$ can be the logistic or hinge loss and the noise amounts to random label flipping.

The generalization error is given by
\begin{align}
    \epsilon_{\mathrm{g}}=\frac{1}{2^{k}} \E_{\boldsymbol{x}, y}\left[\left(\hat{y}\left(\boldsymbol{x}\right)-y\right)^{2}\right]
\end{align}
with $k = 1$ for regression tasks and $k = 2$ for classication tasks.

\paragraph{Dataset}
To mimick a structured dataset, we introduce a block model in which the elements of the inputs $\bs x\in \mathbb R^D$ and the teacher $\bs \beta \in \sR^D$ are sampled from centered Gaussian distributions whose covariances have the following block structure :
\begin{align*}
&\bs x\sim\mathcal{N}(0, \Sigma_x),  &&\Sigma_x = \begin{bmatrix}
\sigx{1} \mathbb I_{\phi_1 D} & 0 & 0\\
0 & \sigx{2} \mathbb I_{\phi_2 D} & 0\\
0 & 0 & \ddots
\end{bmatrix}\\
&\bs \beta \sim\mathcal{N}(0, \Sigma_\beta),  &&\Sigma_\beta = \begin{bmatrix}
\sigb{1} \mathbb I_{\phi_1 D} & 0 & 0 \\
0 & \sigb{2} \mathbb I_{\phi_2 D} & 0\\
0 & 0 & \ddots
\end{bmatrix}.
\end{align*}

%In this model, $\phi_i$ denotes the dimension of the subspace $i$ of input space, $\sigx_i$ denotes its \emph{saliency} (the variance of the inputs in subspace $i$) and $\sigb_i$ denotes its \emph{relevance} (the variance of the teacher weights in subspace $i$).


\paragraph{Main result}

Extending the results of~\cite{gerace2020generalisation}, we use the Replica Method from Statistical Physics~\cite{mezard1987spin,gabrie2019mean} to derive the generalization error in the high-dimensional limit where $N, P, D\to\infty$ with fixed ratios $\gamma=D/P$ and $\alpha=N/P$: 
\begin{align}
    \lim _{N \rightarrow \infty} \epsilon_{g}=\frac{1}{2^k}\E_{\lambda, \nu}\left[\left(f^{0}(\nu)-\hat{f}(\lambda)\right)^{2}\right],
\end{align}
where $\lambda, \nu$ are jointly gaussian with mean zero and covariance :
\begin{align}
    % P(\nu, \lambda) = 
    \Sigma_{\lambda,\nu}=\left(\begin{array}{cc}
    \rho & M \\
    M & Q
    \end{array}\right) \in \sR^{2},
\end{align}
with $\rho= \sum_i \phi_i \sigb{i} \sigx{i}$ and
\begin{align*}
&M= \kappa_{1} \sum_i \sigx{i} m_{s,i}, \quad Q=  \kappa_{1}^2 \sum_i \sigx{i} q_{s,i} +  \kappa_{\star}^{2} q_w  \\
&m_{s,i}=\frac{1}{D} \mathbb E\left[\bs{s}_i \cdot \bs\beta_i\right], \quad q_{s,i}=\frac{1}{D} \mathbb E\left[\bs{s}_i \cdot \bs{s}_i\right], \quad q_{w}=\frac{1}{P} \mathbb E\left[ \bs{w} \cdot \bs{w}\right],
\end{align*}
where $\bs{s}=\frac{1}{\sqrt{P}} F \bs{w} \in \sR^{D}$, and $\bs s_i, \bs \beta_i \in \sR^{\phi_i D}$ denote the orthogonal projections of $\bs s$ and $\bs \beta$ onto subspace $i$.

The role of the activation function is reflected in the constants $\kappa_1, \kappa_\star$ : denoting $r=\sum_i \phi_i \sigx{i}$ and $\xi \sim \mathcal{N}(0,r)$, we have
\begin{align}
\kappa_{1}=\frac{1}{r}\E_\xi[\xi \sigma(\xi)]], \quad &\kappa_{\star}=\sqrt{\E_\xi\left[\sigma(\xi)^{2}\right] - r \kappa_{1}^{2}}
\end{align}

In these equations, the generalization error is expressed in terms or a set of so-called \emph{order parameters} $m_s, q_s, q_w$ whose values can be obtained by solving a set of saddle-point equations as in~\cite{gerace2020generalisation}. These saddle-point equations and their derivation are deferred to the SM.

\paragraph{Square loss regression}

To gain intuition on the formula, we specialize to the square loss regression setup $\ell (x,y) = (x-y)^2$ where $\hat f = f^0 = \text{id}$ and the labels are corrupted by additive noise, i.e. 
\begin{align}
    y^\mu = \frac{\langle\bs \beta ,\bs x^\mu\rangle}{\sqrt D} + \eta, \quad \eta\sim\mathcal{N}(0, \Delta).
\end{align}
The expressions of the test and train error become very informative : 
\begin{align}
    &\epsilon_g = \frac{1}{2}\left(\rho + Q - 2 M \right)\\
    &\epsilon_t = \frac{\epsilon_g + \Delta/2}{(1+V)^2}
\end{align}

Here 
\begin{align}
    &V = \kappa_1^2 \sum_i \sigx{i} v_{s,i} + \kappa_\star^2 v_w\\
    &q_{s,i}=\frac{1}{D} \mathbb V\left[\bs{s}_i \cdot \bs{s}_i\right], \quad q_{w}=\mathbb V\left[\frac{1}{P} \bs{w} \cdot \bs{w}\right]
\end{align}

Note the surprisingly simple relation between the train loss and the test loss. One can invert this expression and write $\epsilon_g = \epsilon_t (1+V)^2 - \Delta/2$, showing that $V$ acts as a variance opening up a generalization gap. 

\paragraph{Square loss classification}

To gain intuition on the formula, we specialize to the square loss classification setup $\ell (x,y) = (x-y)^2$ where $\hat f = f^0 = \text{sign}$ and the labels are corrupted by random label flipping of probability $\Delta$, i.e. 
\begin{align}
    y^\mu = \begin{cases}
    &\text{sign}\left(\frac{\langle\bs \beta ,\bs x^\mu\rangle}{\sqrt D}\right)\quad \text{with probability }1-\Delta\\
    &-\text{sign}\left(\frac{\langle\bs \beta ,\bs x^\mu\rangle}{\sqrt D}\right)\quad \text{with probability }\Delta
    \end{cases}
\end{align}
In this case, the expressions of the train and test error are:
\begin{align}
    &\epsilon_g = \frac{1}{\pi} \cos ^{-1}\left(\frac{M}{\sqrt{\rho Q}}\right)\\
    &\epsilon_t = \frac{1}{2(1+V)^2}\left( \rho + Q - 2 (1- 2 \Delta) M \right)
\end{align}


\section{Strong and weak features model}

\begin{figure*}[htb]
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=.49\linewidth]{figs-rf/{agreement_parameter_wise_te_error_tanh_noise0.0_lamb0.001_regression}.pdf}
    \includegraphics[width=.49\linewidth]{figs-rf/{agreement_sample_wise_te_error_tanh_noise0.0_lamb0.001_regression}.pdf} 
    \caption{Regression}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=.49\linewidth]{figs-rf/{agreement_parameter_wise_te_error_tanh_noise0.0_lamb0.001_classification}.pdf} 
    \includegraphics[width=.49\linewidth]{figs-rf/{agreement_sample_wise_te_error_tanh_noise0.0_lamb0.001_classification}.pdf} 
    \caption{Classification}
    \end{subfigure}
    \caption{\textbf{Anisotropic data strongly affects the double descent curve.} The agreement between theory and numerics is excellent even at moderate size $D=200$ (the vertical bars denote standard deviations over 10 runs). Our analytics allow us to extend far beyond the sizes achievable computationally. He we considered the noiseless setting for $\sigma = \mathrm{Tanh}$, $\lambda=10^{- 3}$. \textit{Left:} parameter-wise profile at $N/D=1$. \textit{Right:} sample-wise profile at $P/D=1$.}
    \label{fig:agreement}
\end{figure*}

\begin{figure*}[htb]
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=.49\linewidth]{figs-rf/{agreement_parameter_wise_te_error_tanh_noise0.3_lamb0.001_regression}.pdf}
    \includegraphics[width=.49\linewidth]{figs-rf/{agreement_sample_wise_te_error_tanh_noise0.3_lamb0.001_regression}.pdf}
    \caption{Regression}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=.49\linewidth]{figs-rf/{agreement_parameter_wise_te_error_tanh_noise0.3_lamb0.001_classification}.pdf}
    \includegraphics[width=.49\linewidth]{figs-rf/{agreement_sample_wise_te_error_tanh_noise0.3_lamb0.001_classification}.pdf}
    \caption{Classification}
    \end{subfigure}
    \caption{\textbf{Irrelevant features can act as regularization.} \textit{Top} : The parameter-wise curve can become non-decreasing in the anisortopic setup. The sample-wise curve exhibits triple descent in the anisoptropic setup, even at signal-to-noise ratio smaller than unity. \textit{Top} : In the classification setting, noise has a weaker effect. We used the same setting as Fig.~\ref{fig:agreement}, but we added noise in the labels, $\Delta=0.4$.}
    \label{fig:agreement-noise}
\end{figure*}

\subsection{Exactness of the main result}
Focusing on the regression case, in Figure~\ref{fig:agreement}, we test the validity of our main result by comparing the analytical predictions of the train and test error with the outcomes of numerical experiments at finite size $D=100$ for $\phi=\phi_1=0.1$ (the small subspace contains 10 features). As can be seen, the agreement is excellent both in the parameter-wise curves where we vary the number of parameters $P$ (left panel) and the sample-wise curves where we vary the number of training samples $N = \alpha P$ (right panel).

\subsection{Impact of structure on learning curves}
Throughout this section, we compare four scenarios. The first is the \emph{isotropic} setup, where $r_x=1$ (blue curves). In the three next, the data is anisotropic. We keep the variance of the inputs and outputs unchanged ($\E \Vert \bs x \Vert = \phi_1 \sigma_{x,1} + \phi_2 \sigma_{x,2}=1$ and $E y^2 = \phi_1 \sigma_{x,1} \sigma_{\beta,1} + \phi_2 \sigma_{x,2}=1 \sigma_{\beta,2}=1$). However, most of the variance of the inputs is concentrated in the first subspace ($r_x=10$). We study three cases for the outputs : (ii) the \emph{easy} case where the salient features are the most relevant ($r_\beta=100$) ; (iii) the \emph{intermediate} case, where all the features have same relevance ; (iv) the \emph{hard} case where the salient features have low relevance ($r_\beta=0.01$) and act as noise.

\paragraph{Structure reduces the effective dimension}

Increasing saliency and relevance of the small subspace effectively makes the task lower-dimensional, therefore easier, albeit in different ways. If most of the task is contained in the small subspace, one could expect the number of parameters or data required to learn to become smaller - this is what we call ``beating the curse of dimensionality". In the regression setup, we see that the onset of learning occurs at the same number of examples ($N=D$) and parameters ($P=D$) for the blue and orange, signalling the RF model is not beating the curse of dimensionality if we only increase the relevance of the parameter $\phi$.

However, if we increase both $r_x$, we see that the test loss starts decreasing earlier, in line with the results of~\cite{ghorbani2020neural}. This can be seen both in the parameter-wise profile (the test loss starts dropping at $P = \phi D$) and in the sample-wise profile (the test loss starts dropping at $N = \phi D$). 

% \begin{figure*}[htb]
%     \centering
%     \begin{subfigure}[b]{\textwidth}	   
%     \includegraphics[width=.49\linewidth]{figs-rf/varying_rphi_parameter_wise_te_error_tanh_noise0.0_lamb0.001_regression}.pdf}
%     \includegraphics[width=.49\linewidth]{figs-rf/varying_rphi_sample_wise_te_error_tanh_noise0.0_lamb0.001_regression}.pdf}
%     \caption{Regression}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}	   
%     \includegraphics[width=.49\linewidth]{figs-rf/varying_rphi_parameter_wise_te_error_tanh_noise0.0_lamb0.001_classification}.pdf}
%     \includegraphics[width=.49\linewidth]{figs-rf/varying_rphi_sample_wise_te_error_tanh_noise0.0_lamb0.001_classification}.pdf}
%     \caption{Classification}
%     \end{subfigure}
%     \caption{\textbf{The size of the blocks determines the onset of learning.} \textit{Left:} parameter-wise profile at $N/D=10^5$. \textit{Right:} sample-wise profile at $N/D=10^5$. We set $\Delta=0, \sigma=\mathrm{Tanh}, \lambda=10^{-3}$.}
%     \label{fig:varying rphi}
% \end{figure*}

\paragraph{Overfitting}
To discuss the overfitting peaks, we use the terminology introduced in~\cite{d2020triple}, and distinguish the linear peaks (those due purely to the noise, which occur at $N_i = \phi_i D$) from the nonlinear peak (that due to the initialization variance, which occur at $N=P$). The nonlinear peak, clearly visible in all figures at $N=P$, only occurs when the data is isotropic (blue and orange curves), whether or not the teacher is concentrated in the small subspace. In other words, anisotropic data distributions mitigate the double descent curve.

However, the phenomenology of the linear peak, which can be seen in the parameter-wise profile, is more complex. We see that the test loss can exhibit zero (blue curve), one (orange curve) or two (red and green curves) linear peaks, located at $N_i = \phi_i D$. This is in line with the empirical findings of~\cite{nakkiran2020optimal,chen2020multiple}.


\section{A case study : more features or more data ?}

\paragraph{A symmetric phase space}

A puzzling observation one can make on the double descent phenomenon is the fact that it appears to occur both parameter-wise and sample-wise. Thus, the number of training parameters $P$ and number of training examples $N$ play similar roles in terms of generalization performance, despite playing opposite roles in terms of capacity (train loss always decreases with $P$ and increases with $N$). In other words, a large model applied to a small dataset gives similar performance to a small model applied to a large dataset.

We test this idea by exploring the full phase-space of the generalization error in Fig.~\ref{fig:phase-space}(a)\footnote{The efficiency of our replica formalism allows to compute the $15\times 15$ values of generalization error in less than a minute.}. In the isotropic setup, we see that the symmetry is exact : the generalization error is unchanged by inverting $P$ and $N$.

Interestingly, this curious symmetry is broken when the data becomes either noisy (panel (b)) or anisotropic (panels (c) and (d)). In this situation, having a lot of data becomes much more useful than having a lot of parameters. In this phase-space view, we also see that the triple descent phenomenon, observed in~\cite{d2020triple} for isotropic regression tasks at high noise, also holds in noiseless classification tasks when the data is anisotropic.

\paragraph{The case of neural networks}

To test whether this disymetrisation of the phase space with noise holds in realistic holds in a more general context, we now turn to neural networks trained on real-world datasets : MNIST and CIFAR10.
To enable an exploration of the phase space at large $N/D$ and $P/D$, we downscale the images to $8\times 8$ pixels, such that $D=64$.
We then train a two-layer fully-connected neural network (with both layers trained) for 300 epochs. We use SGD with momentum 0.9, learning rate 0.01 and batch size 100. We mimick the sign flips of the labels by shuffling the labels with a certain probability. 

The phase spaces are shown in the bottom row of Fig.~\ref{fig:phase-space}. Remarkably, if we define $P$ as the total number of parameters of the two-layer network, the phase space is almost perfectly symmetric when the labels are not shuffled
Remarkably, making the dataset less isotropic in this way also breaks the symmetry in favour of having more data than parameters.

\begin{figure*}[htb]
    \centering
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-rf/{phase_space_te_error_rx1.0_rb1.0_relu_noise0.0_lamb0.001_classification}.pdf}
    \caption{Isotropic, noiseless}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-rf/{phase_space_te_error_rx1.0_rb1.0_relu_noise0.4_lamb0.001_classification}.pdf}
    \caption{Isotropic, $\Delta=0.4$}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-rf/{phase_space_te_error_rx100.0_rb100.0_relu_noise0.0_lamb0.001_classification}.pdf}
    \caption{Anisotropic, $\Delta=0$}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-rf/{phase_space_te_error_rx100.0_rb100.0_relu_noise0.4_lamb0.001_classification}.pdf}
    \caption{Anisoptropic, $\Delta=0.4$}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/MNIST_0.pdf}
    \caption{MNIST, noiseless}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/{MNIST_0.2}.pdf}
    \caption{MNIST, 20\% label noise}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/CIFAR10_0.pdf}
    \caption{CIFAR10, noiseless}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/{CIFAR10_0.2}.pdf}
    \caption{CIFAR10, 20\% label noise}
    \end{subfigure}
    \caption{\textbf{The symmetry of the ($N,P$) phase space vanishes when the data becomes noisy or anisotropic.} \textit{Top:} increasing the anisotropy at $\Delta=0.4$. \textit{Middle:} increasing the noise in the isotropic setup. \textit{Bottom:} results are qualitatively similar for a 2-layer neural network trained on MNIST: as we increase the label noise, the ($N,P$) phase becomes less symmetric.}
    \label{fig:phase-space}
\end{figure*}


To demonstrate this, we plot the phase space in the four scenarios explained above. We see that as the dataset becomes less isotropic, the optimal performance shifts towards the 



==> dfdxcbxrhpmwxgqmtdsvvrxqthrzkvjb/deprecated/spiked.tex <==
\subsection{Effect of anisotropy}

In Figs.~\ref{fig:phase-space},\ref{fig:phase-space-2d}, we show the test error phase space space of the RF model under this particular data distribution. We vary both the correlation parameter $c$ (from left to right) and the alignment of the teacher along the special direction $t^0=\theta^0\cdot\vec1$ (from top to bottom). Fig.~\ref{fig:phase-space} is useful to get a broad qualitative view of the phase space, whereas Fig.~\ref{fig:phase-space-2d} helps to get a more quantitative picture. Note that in the isotropic setup $c=0$ (left panels), the test error is independent of the direction of the teacher, as expected. 

Consider first the case where the teacher is orthogonal to the special direction. In this case, increasing $c$ is detrimental. Indeed when $c$ is close to 1, the data points are completely orthogonal to the teacher: the label is pure noise and the test error never goes below 1 (nothing is learnt). 

When the teacher is perfectly aligned to the special direction, we could expect that aligning the data along the special direction would be beneficial. This is indeed the case when we have little data or little parameters: a dip of low test loss forms. But in the quadrant $N/D>1, P/D>1$, we instead observe a strong overfitting plateau, which merges the linear and nonlinear peaks together. Note that this overfitting occurs even in the linear case and in absence of noise, 

There are two possible explanations for this (which are possible linked). 

The first is the fact that the data lacks diversity. At $c=1$, all the data lies on a line and we can only learn the projection of the teacher along this line.

The second is that since the cosine function varies strongly near $\pi/2$, points which lie are orthogonal to the teacher offer a lot of information (a single point perfectly orthogonal to the teacher uniquely determines the direction of the teacher!), but they are strongly impacted by noise. Having few such points gives a lot of information, but this information is "risky".

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/data_distribution.pdf}
    \caption{Data distribution}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t0_lam0.1_act0.9_noise5.0.pdf}
    \caption{$t^0=0$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t0.5_lam0.1_act0.9_noise5.pdf}
    \caption{$t^0=0.5$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t1_lam0.1_act0.9_noise5.0.pdf}
    \caption{$t^0=1$}
    \end{subfigure}
    \caption{3D phase spaces.}
    \label{fig:phase-space}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t0_lam0.1_act0.9_noise5.0.pdf}
    \caption{$t^0=0$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t0.5_lam0.1_act0.9_noise5_regression.pdf}
    \caption{$t^0=0.5$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t1_lam0.1_act0.9_noise5.0.pdf}
    \caption{$t^0=1$}
    \end{subfigure}
    \caption{2D phase spaces.}
    \label{fig:phase-space-2d}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t0_lam0.1_act0.9_noise0.0.pdf}
    \caption{$t^0=0$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t0.5_lam0.1_act0.9_noise0.pdf}
    \caption{$t^0=0.5$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t1_lam0.1_act0.9_noise0.0.pdf}
    \caption{$t^0=1$}
    \end{subfigure}
    \caption{2D phase spaces.}
    \label{fig:phase-space-2d}
\end{figure}

\subsection{Effect of nonlinearity}

In Fig.~\ref{fig:nonlinearity}, we study the effect of the degree of nonlinearity. We see that in the highly nonlinear case (ReLU), the dip replaces the linear peak at $N=D$, and becomes deeper as we increase $c$. In other words, the network is learning the correlation structure of the data and actually taking profit of it.

In the intermediate case (Tanh), the dip still appears, but it is located before N=D. This makes the triple descent hard to see.

In the linear case, the dip only appears at very high $c$ and is even more shifted the the left.

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t1_lam0.1_act0.5_noise5.0.pdf}
    \caption{r=0.5 (ReLU)}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t1_lam0.1_act0.9_noise5.0.pdf}
    \caption{r=0.9 (Tanh)}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t1_lam0.1_act1_noise5.0.pdf}
    \caption{r=1 (Linear)}
    \end{subfigure}
    \caption{Effect of degree of nonlinearity}
    \label{fig:nonlinearity}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t1_lam0.1_act0.5_noise5.0.pdf}
    \caption{r=0.5 (ReLU)}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t1_lam0.1_act0.9_noise5.0.pdf}
    \caption{r=0.9 (Tanh)}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t1_lam0.1_act1.0_noise5.0.pdf}
    \caption{r=1 (Linear)}
    \end{subfigure}
    \caption{Effect of degree of nonlinearity}
    \label{fig:nonlinearity-2d}
\end{figure}

\subsection{Effect of noise}

In Fig.~\ref{fig:snr}, we study the effect of the SNR. We see that in the noiseless case, adding some correlation revives overfitting, even the linear peak.

In the intermediate case (Tanh), the dip still appears, but it is located before N=D.

In the linear case, the dip is harder to see.

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t1_lam0.1_act0.9_noise0.0.pdf}
    \caption{SNR = $\infty$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t1_lam0.1_act0.9_noise0.5.pdf}
    \caption{SNR = 2}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/3D_phase_space_t1_lam0.1_act0.9_noise5.0.pdf}
    \caption{SNR = 0.2}
    \end{subfigure}
    \caption{Effect of SNR}
    \label{fig:snr}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t1_lam0.1_act0.9_noise0.0.pdf}
    \caption{SNR = $\infty$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t1_lam0.1_act0.9_noise0.5.pdf}
    \caption{SNR = 2}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=\linewidth]{figs_spiked/phase_space_t1_lam0.1_act0.9_noise5.0.pdf}
    \caption{SNR = 0.2}
    \end{subfigure}
    \caption{Effect of SNR}
    \label{fig:snr-2d}
\end{figure}


\subsection{Consequence on optimal regularization}

It is expected that when the input-output covariance becomes anisotropic, the optimal regularization parameter can become negative in the overparametrized regime. This is indeed what we observe in Fig.~\ref{fig:regularization}. 

As we increase the anisotropy of the input data by increasing $c$, we see that the test error vs $\gamma$ curve changes significantly. In particular, it strongly depends on whether the teacher is correlated or not with the special direction. When the teacher is indeed aligned, we start to see a negative optimal $\gamma$ as in Fig.3 of \cite{wu2020optimal}. Instead when the teacher is anti-aligned it is better to regularize.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs_spiked/regularization.pdf}
    \caption{Test loss vs regularization}
    \label{fig:regularization}
\end{figure}

\subsection{Derivation}

\section{Spiked covariance}

We consider the RF model in the correlated input data setting: $x\sim\mathcal{N}(0,\Sigma)$ with $\Sigma_{ij} = \delta_{ij}+c (1-\delta_{ij})$. This amounts to squishing the input data along a special direction: the vector $\vec 1= (1~1...)^\top$ (see top panel of Fig.~\ref{fig:phase-space} for an illustration).

The replicated gaussian equivalence theorem stated in~\cite{gerace2020generalisation} establishes that the following variables
\begin{align}
    \lambda^{a}=\frac{1}{\sqrt{p}} \boldsymbol{w}^{a} \cdot \sigma(\boldsymbol{\Theta} \boldsymbol{x}) \in \sR, \quad \nu=\frac{1}{\sqrt{d}} \boldsymbol{x} \cdot \boldsymbol{\theta}^{0} \in \sR
\end{align}
Are jointly gaussian:
\begin{align}
&\E\left[\lambda^{a} \lambda^{b}\right]=\frac{\kappa_{\star}^{2}}{p} \boldsymbol{w}^{a} \cdot \boldsymbol{w}^{b}+\frac{\kappa_{1}^{2}}{d} \left((1-c) \boldsymbol{s}^{a} \cdot \boldsymbol{s}^{b} + c\sum_i \bs s_i^a \sum_j \bs s_j^a  \right)\\
&\E\left[\nu^{2}\right]=\frac{1}{d}\left\|\boldsymbol{\theta}^{0}\right\|^{2}\\
&\E\left[\lambda^{a} \nu\right]=\frac{\kappa_{1}}{d} \left((1-c)\boldsymbol{s}^{a} \cdot \boldsymbol{\theta}^{0} + c \sum_i \bs s_i^a \sum_j \bs \theta^0 \right)\\
&\boldsymbol{s}^{a}=\frac{1}{\sqrt{p}} F \boldsymbol{w}^{a} \in \sR^{d}, \quad a=1, \cdots, r \\
&\kappa_{0}=\E_{z}[\sigma(z)], \quad \kappa_{1}=\E_{z}[z \sigma(z)], \quad \kappa_{\star}=\E_{z}\left[\sigma(z)^{2}\right]-\kappa_{0}^{2}-\kappa_{1}^{2}
\end{align}

Here we see that new order parameters intervene: $\sum_i \bs s^a_i = \frac{1}{\sqrt{d}}\bs s^a\cdot\vec1$ and $\sum_i \bs \theta^0_i = \bs \theta^0\cdot\vec1$, in other words the alignment of the student and the teacher with respect to the special direction $\vec 1$.

But in a more compact form,
\begin{align}
(\lambda^a, \nu) \sim \mathcal{N}(0,\Sigma), \quad 
\Sigma^{a b}=\left(\begin{array}{cc}
\rho & M^{a} \\
M^{a} & Q^{a b}
\end{array}\right) \in \sR^{(r+1) \times(r+1)}
\end{align}

\begin{align}
&\rho=\frac{1}{d}\left\|\boldsymbol{\theta}^{0}\right\|^{2}, M^{a}=\kappa_{1} \left((1-c) m_{s}^{a} + c t^0 t_s^a\right), \quad Q^{a b}=\kappa_{\star}^{2} \left((1-c) q_w^{ab} + ct_s^a t_s^b  \right)\\
&m_{s}^{a}=\frac{1}{d} \boldsymbol{s}^{a} \cdot \boldsymbol{\theta}^{0}, \quad q_{s}^{a b}=\frac{1}{d} \boldsymbol{s}^{a} \cdot \boldsymbol{s}^{b}, \quad q_{w}^{a b}=\frac{1}{p} \boldsymbol{w}^{a} \cdot \boldsymbol{w}^{b}\\
&t^a_s = \frac{1}{d} \bs s^a \cdot \vec 1, \quad t^0 = \frac{1}{d} \bs \theta^0 \cdot \vec 1,
\end{align}

The calculations follow through in a similar way:
\begin{align}
\begin{aligned}
f_{\beta}\left(\left\{\boldsymbol{x}^{\mu}, y^{\mu}\right\}\right)&=-\frac{1}{p} \log \gZ_{\beta}\\
\E_{\left\{\boldsymbol{x}^{\mu}, y^{\mu}\right\}} \gZ_{\beta}^{r}&=\int \frac{\dd \rho \dd \hat{\rho}}{2 \pi} \int \prod_{a=1}^{r} \frac{\dd m_{s}^{a} \dd \hat{m}_{s}^{a}}{2 \pi} \int \prod_{1 \leq a \leq b \leq r} \frac{\dd q_{s}^{a b} \dd \hat{q}_{s}^{a b}}{2 \pi} \frac{\dd q_{w}^{a b} \dd \hat{q}_{w}^{a b}}{2 \pi} e^{p \Phi^{(r)}}\\
\Phi^{(r)}&=- \gamma \rho \hat{\rho} - \gamma t^0 \hat{t^0}-\gamma \sum_{a=1}^{r} m_{s}^{a} \hat{m}_{s}^{a} -\gamma \sum_{a=1}^{r} t_{s}^{a} \hat{t}_{s}^{a}-\sum_{1 \leq a \leq b \leq r}\left(\gamma q_{s}^{a b} \hat{q}_{s}^{a b}+q_{w} \hat{q}_{w}\right)+\alpha \Psi_{y}^{(r)}\left(\rho, m_{s}^{a}, q_{s}^{a b}, q_{w}^{a b}\right) \\
&+\Psi_{w}^{(r)}\left(\hat{\rho}, \hat{m}_{s}^{a}, \hat{q}_{s}^{a b}, \hat{q}_{w}^{a b}\right)
\end{aligned}
\end{align}

Once we decouple the replicas, we obtain as order parameters
\begin{align}
    M=\kappa_{1} \left((1-c) m_{s} + c t^0 t_s\right), \quad Q=\kappa_{\star}^{2} q_{w}+\kappa_{1}^{2} \left((1-c)q_{s} + c t_s^2\right), \quad R=\kappa_{\star}^{2} r_w + \kappa_1^2 \left((1-c)r_{s} + c t_s^2\right)
\end{align}
Which allows to compute $\Psi_y$.

As for $\Psi_w$, we must take into account the new order parameter:
\begin{align}
    \Psi_{w}=\lim _{p \rightarrow \infty} \frac{1}{p} \E_{\xi, \eta, \theta^{0}} \log \int_{\sR^{d}} \operatorname{d} \boldsymbol{s} P_{s}(\boldsymbol{s} ; \eta) e^{-\frac{\hat{V}_{s}}{2}\|\boldsymbol{s}\|^{2}+\left(\sqrt{\hat{q}_{s}} \xi \mathbf{1}_{d}+\hat{m}_{s} \boldsymbol{\theta}^{0} + \hat t_s \vec 1\right)^{\top} \boldsymbol{s}}
\end{align}

We can see that this amounts to adding a new teacher term in the direction $\vec 1$: $$\hat m_s \theta^0\to \hat m_s \theta^0+ \hat t_s \vec 1$$ 

Therefore the only change will concern terms of the form $\hat m_s^2 \to \hat m_s^2 + \hat t_s^2 + 2 \hat m_s \hat t_s t^0$

The saddle-point equations become
\begin{align}
\left\{\begin{array}{ll}
\hat{r}_{s}=-2 \frac{\alpha}{\gamma} \partial_{r_{s}} \Psi_{y}(R, Q, M) & \quad r_{s}=-\frac{2}{\gamma} \partial_{\hat{r}_{s}} \Psi_{w}\left(\hat{r}_{s}, \hat{q}_{s}, \hat{m}_{s}, \hat{t}_{s}, \hat{r}_{w}, \hat{q}_{w}\right) \\
\hat{q}_{s}=-2 \frac{\alpha}{\gamma} \partial_{q_{s}} \Psi_{y}(R, Q, M) & q_{s}=-\frac{2}{\gamma} \partial_{\hat{q}_{s}} \Psi_{w}\left(\hat{r}_{s}, \hat{q}_{s}, \hat{m}_{s}, \hat{t}_{s}, \hat{r}_{w}, \hat{q}_{w}\right) \\
\hat{m}_{s}=\frac{\alpha}{\gamma} \partial_{m_{s}} \Psi_{y}(R, Q, M) & m_{s}=\frac{1}{\gamma} \partial_{\hat{m}_{s}} \Psi_{w}\left(\hat{r}_{s}, \hat{q}_{s}, \hat{m}_{s}, \hat{t}_{s}, \hat{r}_{w}, \hat{q}_{w}\right) \\
\hat{t}_{s}=\frac{\alpha}{\gamma} \partial_{t_{s}} \Psi_{y}(R, Q, M) & t_{s}=\frac{1}{\gamma} \partial_{\hat{t}_{s}} \Psi_{w}\left(\hat{r}_{s}, \hat{q}_{s}, \hat{m}_{s}, \hat{t}_{s}, \hat{r}_{w}, \hat{q}_{w}\right)\\
\hat{r}_{w}=-2 \alpha \partial_{r_{w}} \Psi_{y}(R, Q, M) & r_{w}=-2 \partial_{\hat{r}_{w}} \Psi_{w}\left(\hat{r}_{s}, \hat{q}_{s}, \hat{m}_{s}, \hat{t}_{s}, \hat{r}_{w}, \hat{q}_{w}\right) \\
\hat{q}_{w}=-2 \alpha \partial_{q_{w}} \Psi_{y}(R, Q, M) & q_{w}=-2 \partial_{\hat{q}_{w}} \Psi_{w}\left(\hat{r}_{s}, \hat{q}_{s}, \hat{m}_{s}, \hat{t}_{s}, \hat{r}_{w}, \hat{q}_{w}\right)
\end{array}\right.
\end{align}

\begin{align}
\left\{\begin{array}{l}
V_{s}=\frac{1}{\hat{V}_{s}}\left(1-z g_{\mu}(-z)\right) \\
q_{s}=\frac{\hat m_s^2 + \hat t_s^2 + 2 \hat m_s \hat t_s t^0+\hat{q}_{s}}{\hat{V}_{s}^{2}}\left[1-2 z g_{\mu}(-z)+z^{2} g_{\mu}^{\prime}(-z)\right]-\frac{\hat{q}_{w}}{\left(\beta \lambda+\hat{V}_{w}\right) \hat{V}_{s}}\left[-z g_{\mu}(-z)+z^{2} g_{\mu}^{\prime}(-z)\right] \\
m_{s}=\frac{\hat{m}_{s} + \hat t_s t^0}{\hat{V}_{s}}\left(1-z g_{\mu}(-z)\right) \\
t_{s}=\frac{\hat{t}_{s} + \hat m_s t^0}{\hat{V}_{s}}\left(1-z g_{\mu}(-z)\right) \\
V_{w}=\frac{\gamma}{\beta \lambda+\hat{V}_{w}}\left[\frac{1}{\gamma}-1+z g_{\mu}(-z)\right] \\
q_{w}=\gamma \frac{\hat{q}_{w}}{\left(\beta \lambda+\hat{V}_{w}\right)^{2}}\left[\frac{1}{\gamma}-1+z^{2} g_{\mu}^{\prime}(-z)\right]+\frac{\hat m_s^2 + \hat t_s^2 + 2 \hat m_s \hat t_s t^0+\hat{q}_{s}}{\left(\beta \lambda+\hat{V}_{w}\right) \hat{V}_{s}}\left[-z g_{\mu}(-z)+z^{2} g_{\mu}^{\prime}(-z)\right]
\end{array}\right.
\end{align}

\begin{align}
\left\{\begin{array}{l}
\hat{V}_{s}^{\infty}=(1-c)\frac{\alpha \mu_{1}^{2}}{\gamma} \E_{\xi}\left[\int_{\sR} \dd y \gZ_{y}^{0} \frac{\partial_{\omega} \eta}{V^{\infty}}\right] \\
\hat{q}_{s}^{\infty}=(1-c)\frac{\alpha \mu_{1}^{2}}{\gamma} \E_{\xi}\left[\int_{\sR} \dd y \gZ_{y}^{0}\left(\frac{\eta-\omega}{V^{\infty}}\right)^{2}\right] \\
\hat{m}_{s}^{\infty}=(1-c)\frac{\alpha \mu_{1}}{\gamma} \E_{\xi}\left[\int_{\sR} \dd y \partial_{\omega} \gZ_{y}^{0}\left(\frac{\eta-\omega}{V^{\infty}}\right)\right] \\
\hat{t}_{s}^{\infty}=\frac{2c}{1-c} t^0 \hat m_s\\
\hat{V}_{w}^{\infty}=\alpha \mu_{\star}^{2} \E_{\xi}\left[\int_{\sR}^{\infty} \dd y \gZ_{y}^{0} \frac{\partial_{\omega} \eta}{V^{\infty}}\right] \\
\hat q_s^\infty=\alpha \mu_{\star}^{2} \E_{\xi}\left[\int_{\sR} \dd y \gZ_{y}^{0}\left(\frac{\eta-\omega}{V^{\infty}}\right)^{2}\right]
\end{array}\right.
\end{align}

The test error reads 
\begin{align}
    \epsilon_g = \rho + Q - 2M
\end{align}




==> dfdxcbxrhpmwxgqmtdsvvrxqthrzkvjb/deprecated/strong_weak.tex <==
\subsection{Effect of anisotropy}

We recall that the anisotropy of the strong and weak features model is controlled by three parameters: $\lambda_i, \phi_i, \beta_i$ which respectively denote the strength, size and projected norm of the teacher in each of the eigenspace $i$.




\begin{figure}
    \centering
    \begin{subfigure}[b]{.32\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/sample_wise_act0.99_noise0.0_ds_(0.01, 0.99)_regression.pdf}
    \caption{$\mathrm{SNR}=\infty$}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/sample_wise_act0.99_noise0.5_ds_(0.01, 0.99)_regression.pdf}
    \caption{$\mathrm{SNR}=2$}
    \end{subfigure}    \begin{subfigure}[b]{.32\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/sample_wise_act0.99_noise5.0_ds_(0.01, 0.99)_regression.pdf}
    \caption{$\mathrm{SNR}=0.2$}
    \end{subfigure}
    \caption{Effect of the anisotropy on the test error}
    \label{fig:strengths}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs_strong_weak/sample_wise_act0.99_noise5.0_ds_(0.4, 0.3, 0.2, 0.1)_regression.pdf}
    \caption{Multi-block covariance}
    \label{fig:strengths}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/3D_phase_space_ds_(0.01, 0.99)_cs_(0.01, 1.0)_betas_(0.01, 1.0)_act0.99_noise0.0_regression.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/3D_phase_space_ds_(0.01, 0.99)_cs_(0.01, 1.0)_betas_(1.0, 0.01)_act0.99_noise0.0_regression.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/3D_phase_space_ds_(0.01, 0.99)_cs_(1.0, 0.01)_betas_(0.01, 1.0)_act0.99_noise0.0_regression.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/3D_phase_space_ds_(0.01, 0.99)_cs_(1.0, 0.01)_betas_(1.0, 0.01)_act0.99_noise0.0_regression.pdf}
    \end{subfigure}

    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/3D_phase_space_ds_(0.01, 0.99)_cs_(0.01, 1.0)_betas_(0.01, 1.0)_act0.99_noise5.0_regression.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/3D_phase_space_ds_(0.01, 0.99)_cs_(0.01, 1.0)_betas_(1.0, 0.01)_act0.99_noise5.0_regression.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/3D_phase_space_ds_(0.01, 0.99)_cs_(1.0, 0.01)_betas_(0.01, 1.0)_act0.99_noise5.0_regression.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs_strong_weak/3D_phase_space_ds_(0.01, 0.99)_cs_(1.0, 0.01)_betas_(1.0, 0.01)_act0.99_noise5.0_regression.pdf}
    \end{subfigure}
    \caption{3D phase spaces.}
    \label{fig:phase-spaces-strengths}
\end{figure}

\subsection{Effect of regularization}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs_strong_weak/regularization.pdf}
    \caption{Test loss vs regularization}
    \label{fig:regularization}
\end{figure}

==> dfdxcbxrhpmwxgqmtdsvvrxqthrzkvjb/main_text.tex <==
\section{Introduction}

Despite their remarkable achievements over the past decade~\cite{krizhevsky2012imagenet, lecun2015deep,hinton2012deep,sutskever2014sequence}, deep neural networks continue to puzzle rigorous understanding by their astonishing generalization capacities~\cite{zhang2016understanding,neyshabur2018towards,advani2020high}. On one hand, classical wisdom says that a learning model should have just the right number of parameters to learn from a dataset without overfitting it. On the other hand, recent years have seen the emergence of massively overparametrized models~\cite{zagoruyko2016wide,brown2020language}, which manage to generalize well, somehow avoiding the pitfall of overfitting. 

Various works have given evidence of a double descent curve in deep learning~\cite{advani2020high,spigler2019jamming,belkin2018reconciling,geiger2020scaling}, whereby the test error first decreases as the number of parameters increases, then peaks, then decreases again monotonically. The overfitting peak occurs at the \emph{interpolation threshold} where training error vanishes, and is well-studied in the statistical physics literature~\cite{opper1996statistical,engel2001statistical,krzakala2007landscape,franz2016simplest,geiger2019jamming}. %More recently, it was shown to be related to a sharp increase in the variance of the estimator \cite{geiger2019jamming,d2020double,geiger2020scaling,jacot2020implicit}.

A puzzling observation one can make on the double descent phenomenon is the fact that it appears to occur both parameter-wise and sample-wise~\cite{nakkiran2019deep,nakkiran2019more}. Thus, the number of training parameters $P$ and the number of training examples $N$ play similar roles in generalization performance, being both beneficial, despite playing opposite roles in terms of fitting performance (train loss decreases with $P$ and increases with $N$). In other words, a large model applied to a small dataset happens to give similar test loss to a small model applied to a large dataset. 

This observation is illustrated in Fig.~\ref{fig:phase-space-1}, where we show the train and test error of two-layer fully-connected networks on a downsampled version of CIFAR10. Both quantities are plotted in an $(N, P)$-diagram as a function of the numbers of training samples $N$ and parameters $P$. 
The train error increases with $N$ and decreases with $P$, vanishing at the interpolation threshold for $P$ at a level slightly above $N$. However, the test error decreases when increasing either $N$ or $P$, and the ``generalization phase space" is, in fact, more or less symmetric with respect to the $N=P$ line.

Generally speaking, generalization is allowed by the underlying structure of data. One aspect of data structure is the distribution of inputs: MNIST and CIFAR10 have same number of classes and images, yet generalization is harder for CIFAR10 because the images are more complex. The other aspect of structure is the rule between inputs and outputs: a random labelling of CIFAR10 can be learned by a neural network but offers no possibility of generalization \cite{zhang2016understanding}.  Characterizing the structure of real-world data involves studying the interplay between these two aspects. In this direction, simple, interpretable models of structured data can prove useful to understand what underlies the behaviour of the generalization phase space outlined above. 

\paragraph{Setting} In this work we present a solvable model of learning which enables us to:
\begin{itemize}
    \item[(i)] vary $P$ and $N$ independently; % $D$;
    \item[(ii)] analyze classification tasks; %, as well;
    \item[(iii)] strudy the effect of data structure. 
\end{itemize}

Many works have studied the double descent curve from an analytical point of view~\cite{krogh1992generalization,opper1996statistical,engel2001statistical,hastie2019surprises,nakkiran2020optimal}, yet to the best of our knowledge, none fulfils these three conditions simultaneously. For instance, 
linear models applied to regression problems with i.i.d. Gaussian inputs, which is a commonly analyzed setup, violates each of our three requirements. 

To satisfy \textit{(i)}, we consider a random feature model~\cite{rahimi2008random}, which was shown to exhibit double descent in~\citet{mei2019generalization}. To satisfy \textit{(ii)}, we follow the lines of~\cite{gerace2020generalisation} and use an approach from statistical physics, enabling to generalize the result of~\cite{mei2019generalization} to any convex loss function, as long as the labels are generated by a linear ground truth, i.e. $y=f^0(\bs \beta\cdot \bs x)$ with $\bs \beta \in \sR^D$ a teacher weight vector. 
Finally, to satisfy \textit{(iii)}, we introduce a block model in which the input space is subdivided into various subspaces with different variances ({\it saliency}) and different correlation ({\it relevance}) with the teacher vector $\bs \beta$. This model was studied for linear regression under the name of \textit{strong and weak features model}~\cite{richards2020asymptotics}. 


\begin{figure}[t!]
\centering
    \begin{subfigure}[b]{.49\columnwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/train_error_CIFAR10_pca0_noise0.pdf}
    \caption{Train error}
    \end{subfigure}
    \begin{subfigure}[b]{.49\columnwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_CIFAR10_pca0_noise0.pdf}
    \caption{Test error}
    \end{subfigure}
    \caption{\textbf{The generalization phase space of CIFAR10: number of parameters and training examples play opposite roles in terms of train error but similar roles in terms of generalization.} We trained 2-layer ReLU networks of varying width on CIFAR10, downscaled to $D=10\times 10$ images. $N$ is the number of examples in the training set and $P$ denotes the total number of parameters of the network. \textit{Left:} Train error at convergence. \textit{Right:} Test error at convergence. The phase space is almost symmetric along the line $N=P$: inverting $P$ and $N$ reaches similar test error.}
    \label{fig:phase-space-1}
\end{figure}


\paragraph{Contributions}
Our main analytical contribution is the expression of the generalization error of a random feature model trained on data generated by the strong and weak features model, in the limit where the input dimension $D$, the number of training examples $N$ and the number of parameters $P$ are sent to infinity with their ratios fixed. Our analysis is valid both for regression and classification tasks. We confirm numerically that the asymptotic prediction matches simulations even at moderately large sizes. 

This allows us to study analytically the effect of the data anisotropy on the double descent curves. We show in particular that salient relevant features allow the model to ``beat the curse of dimensionality", whereas salient irrelevant features can act as a form of regularization.

We then investigate the generalization phase space in the same model. In the case of isotropic noiseless data, we observe a quasi-symmetric phase space. We find that noise in the labels or irrelevant features in the inputs tends to make the phase space less symmetric in favor of more data rather than more parameters. Finally, we present numerical investigations of the phase space for two-layer networks trained on MNIST and CIFAR10, and observe a similar phenomenology, demonstrating the relevance of the model considered.

\paragraph{Reproducibility}
We provide an open-source implementation of our experiments. It is available at \url{https://github.com/sdascoli/strong-weak}.

\paragraph{Related Work}

Although most theoretical studies of generalization focus on structureless data, a few exceptions exist. The strong and weak features model has recently been studied in the context of least-squares regression, both empirically~\cite{nakkiran2020optimal} and theoretically~\cite{dobriban2015high,wu2020optimal,richards2020asymptotics}. Several intriguing observation emerge in strongly anisotropic setup: (i) several overfitting peaks can be seen ~\cite{nakkiran2020optimal,chen2020multiple}; (ii) the optimal ridge regularization parameter $\gamma$ can become negative~\cite{wu2020optimal,kobak2019optimal}, as it becomes helpful to encourage the weights to have very different magnitudes; (iii) extra features acting as pure noise can actually play a beneficial role by inducing some implicit regularization~\cite{richards2020asymptotics}.

The strong and weak features model also includes the setup studied in~\citet{ghorbani2020neural}, called the spiked covariates model. It involves a small block of size $D^{\eta}$ scaling polynomially in the input dimension ($\eta < 1$) and a large ``junk" block with no correlation with the labels. The question is then: can kernel methods learn to discard the junk features, hence ``beat the curse of dimensionality" in the way neural networks do? The answer was shown to depend on the strength of the junk features: when the variance of these features small, they are not problematic and the kernel method ignores them, effectively learning a task of effective dimensionality $D^{\eta} \ll D$.

More general models for the structure of data were considered in other works. In the special case of random Fourier Feature regression, \citet{liao2020random} derived the train and test error for a general input distribution. \citet{canatar2020statistical} achieved a similar result in the non-parametric setting of kernel regression, which can be viewed as the limiting case of random feature regression when the number of random features $P$ goes to infinity. 
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
%Add these for the ArXiv Version!!!!
%\cite{jacot2020implicit}
%\cite{jacot2020kernel}
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%

The few works studying classification analytically have mostly focused on linear models, trained on linearly separable data~\cite{montanari2019generalization,chatterji2020finite,liang2020precise} or gaussian mixtures~\cite{deng2019model,mignacco2020role}. One of the challenges in classification (in comparison to regression) is the large set of available loss functions~\cite{kini2020analytic,muthukumar2020classification}. In particular, the choice of the loss impacts the location of the interpolation threshold. A notable exception is~\citet{gerace2020generalisation}, on which our paper builds. Using tools from statistical mechanics, the authors were able to derive the generalization loss of random features model for \textit{any} loss function, yet their results focus on isotropic data.

In a more realistic deep learning setup, \citet{li2019towards} studied the effect of ``hard-to-fit, easy-to-generalize" features, which are very akin to our strong and weak features model. They show that large learning rates favor learning easy-to-fit, hard-to-generalize features (what we would call highly salient but little relevant). In contrast, a small learning rate does the opposite, motivating the use of learning rate decay.


\begin{figure*}[!ht]
    \centering
    \includegraphics[width=.3\linewidth]{RF.pdf}
    \includegraphics[width=.45\linewidth]{Data.pdf}
    \caption{\textit{Left:} Random feature model considered here, which can be viewed as a two-layer networks where only the second layer is trained. \textit{Right:} Strong and weak features model considered here. Input space is decomposed into two subspaces, a \emph{salient} one with strong variance $\sigma_{x,1}$ and the other with smaller variance $\sigma_{x,2}$. We can adjust the \emph{relevance} of both subspaces by adjusting the variance of the teacher $\bs \beta$ which they contain. The task is easy when $\sigma_{\beta,1}>\sigma_{\beta,2}$, and hard in the opposite case.}
    \label{fig:RF}
\end{figure*}

\section{A solvable model of data structure}

To explore the properties of the generalization phase space, we focus on the random features model\footnote{This model is akin to the so-called lazy learning regime of neural networks where the weights stay close to their initial value~\cite{jacot2018neural}: assuming $f_{\theta_0}\!=\!0$, we have $f_{\theta}({\bf x}) \approx \nabla_{\theta}f_{\theta}({\bf x})|_{\theta\!=\!\theta_0} \cdot (\theta-\theta_0)$~\cite{chizat2018note}. In other words, lazy learning amounts to a linear fitting problem with a random feature vector $\left.\nabla_{\theta}f_{\theta}({\bf x})\right|_{\theta\!=\!\theta_0}$.}  introduced in \citet{rahimi2008random}.
Using tools from statistical physics, we derive the generalization error in a teacher-student scenario, including the strong and weak features model of structured data. 
Albeit non-rigorous in a strict mathematical sense, these methods are considered exact in theoretical physics and have been influential to statistical learning theory since the 80s, see \citet{gabrie2019mean} and \citet{bahri2020review} for recent reviews. Moreover, several of their conjectures have been proven exact in the last decade \cite{barbier2019optimal, aubin2018committe, gabrie2018entropy,  goldt2020gaussian}.

\paragraph{Random feature model}
The random features model can be viewed as a two-layer neural network whose first layer is fixed random matrix containing $P$ random features $\{\bs F_i\in\mathbb R^D\}_{i=1\ldots P}$:
\begin{equation}
    \hat y_\mu = \hat f\left(\sum_{i=1}^P\bs w_i \sigma\left(\frac{\bs F_i \cdot \bs x_\mu}{\sqrt{D}}\right)\right)\equiv \hat f\left(\bs w\cdot \bs z_\mu \right),
\end{equation} 
where $\sigma(\cdot)$ is a pointwise activation function, $\hat f$ is an output function and we introduced the notation $\bs z_\mu \in \sR^P$.
Elements of $\bs F$ are drawn i.i.d from $\mathcal{N}(0,1)$.  The labels are given by a linear ground truth, modulated by an output function $f^0$ and possibly corrupted by noise through a probabilistic channel $\gP$:
\begin{equation}
    \label{eq:teacher-def}
    y_\mu \sim \gP \left( \cdot \left\vert  f^0\left(\frac{\bs \beta\cdot\bs x_\mu}{\sqrt D}\right)\right.\right).
\end{equation}

The second layer weights, i.e. the elements of $\bs w \in \sR^P$, are trained by minimizing an $\ell_2$-regularized loss on $N$ training examples $\{\bs x_\mu\in\R^D\}_{\mu=1\ldots N}$ :
\begin{align}
    \label{eq:ridge-estimator}
    \hat{\boldsymbol{w}}&=\underset{\boldsymbol{w}}{\operatorname{argmin}} \left[\epsilon_t(\bs w) \right],\\
    \epsilon_t(\bs w) &= \sum_{\mu=1}^{N} \ell\left(y^{\mu}, \bs w \cdot \bs z_\mu \right)+\frac{\lambda}{2}\|\boldsymbol{w}\|_{2}^{2}.
\end{align}
We consider both regression tasks, where $\hat f = f^0 = \text{id}$, and binary classification tasks, $\hat f = f^0 = \text{sign}$. In the first case, $\ell$ is the square loss and the noise is additive. In the second case, $\ell$ can be any type of loss (square, hinge, logistic) and the noise amounts to random label flipping.

The generalization error is given by
\begin{align}
    \epsilon_{g}=\frac{1}{2^{k}} \E_{\boldsymbol{x}, y}\left[\left(\hat{y}\left(\boldsymbol{x}\right)-y\right)^{2}\right]
\end{align}
with $k = 1$ for regression tasks (mean-square error) and $k = 2$ for binary classification tasks (zero-one error).

\paragraph{Strong and weak features model}
% To mimic a structured dataset, 
To impose structure on the dataset,
we introduce a block model in which the elements of the inputs $\bs x\in \mathbb R^D$ and the teacher $\bs \beta \in \sR^D$ are sampled from centered Gaussian distributions whose covariances have the following block structure :
\begin{align*}
&\bs x\sim\mathcal{N}(0, \Sigma_x),  &&\Sigma_x = \begin{bmatrix}
\sigx{1} \mathbb I_{\phi_1 D} & 0 & 0\\
0 & \sigx{2} \mathbb I_{\phi_2 D} & 0\\
0 & 0 & \ddots
\end{bmatrix},\\
&\bs \beta \sim\mathcal{N}(0, \Sigma_\beta),  &&\Sigma_\beta = \begin{bmatrix}
\sigb{1} \mathbb I_{\phi_1 D} & 0 & 0 \\
0 & \sigb{2} \mathbb I_{\phi_2 D} & 0\\
0 & 0 & \ddots
\end{bmatrix}.
\end{align*}

Although our theory is valid for an arbitrary number of blocks, we will focus for interpretability on the special case where we only have two blocks of sizes $\phi_1 D$ and $\phi_2 D$, with $\phi_1 + \phi_2 = 1$ (see Fig.~\ref{fig:RF}). We will typically be interested in the strongly anisotropic setup where the first subspace is much smaller $\phi_1 \ll 1$, but potentially has higher \emph{saliency} $r_x = \sigx{1}/ \sigx{2} \gg 1$ and higher \emph{relevance} $r_\beta = \sigb{1}/ \sigb{2} \gg 1$. 
%This strong and weak features model is related to the setup studied by \citet{ghorbani2020neural} where the size of the small relevant subspace scales polynomially in the total dimension of input, whereas here, the scaling is linear.

\paragraph{Main analytical result}
Using the replica method from statistical physics~\cite{mezard1987spin} and the Gaussian Equivalence Theorem~\cite{el2010spectrum,mei2019generalization,goldt2020gaussian,hu2020universality}, we derive the generalization error in the high-dimensional limit where $D, N$ and $P\to\infty$ with fixed ratios.
Our result extends the result of~\citet{gerace2020generalisation} for isotropic data to anisotropic data; we additionally derive the effect of label flipping.

The asymptotic generalization error is given by 
\begin{align}
    \lim _{N \rightarrow \infty} \epsilon_{g}=\frac{1}{2^k}\E_{\lambda, \nu}\left[\left(f^{0}(\nu)-\hat{f}(\lambda)\right)^{2}\right],
\end{align}
where $\lambda, \nu$ are jointly Gaussian scalars with mean zero and covariance:
\begin{align}
    % P(\nu, \lambda) = 
    \Sigma_{\lambda,\nu}=\left(\begin{array}{cc}
    \rho & M \\
    M & Q
    \end{array}\right) \in \sR^{2},
\end{align}
with 
\begin{align}
&\rho = \sum_i \phi_i \sigb{i} \sigx{i}, \quad M= \kappa_{1} \sum_i \sigx{i} m_{s,i}, \notag\\
&\text{ and } \quad Q = \kappa_{1}^2 \sum_i \sigx{i} q_{s,i} +  \kappa_{\star}^{2} q_w.
\label{eq:replica-M-Q}
\end{align}
where the parameters $\kappa_1, \kappa_\star$ are related to the activation function: denoting $r=\sum_i \phi_i \sigx{i}$ and $\xi \sim \mathcal{N}(0,r)$, one has
\begin{align}
\kappa_{1}=\frac{1}{r}\E_\xi[\xi \sigma(\xi)]], \quad &\kappa_{\star}=\sqrt{\E_\xi\left[\sigma(\xi)^{2}\right] - r \kappa_{1}^{2}}.
\end{align}
Besides these constants and the ones defining the data structure ($\phi_i ,\sigb{i} ,\sigx{i}$), the key ingredients to obtain the covariance elements in (\ref{eq:replica-M-Q}) are the so-called \emph{order parameters} $m_s, q_s, q_w$. They correspond to the high-dimensional limit of the following overlaps:
\begin{align*}
m_{s,i} &=\lim_{D\to\infty}\frac{1}{D} \E_\mathcal{P}\left[\bs{s}_i \cdot \bs\beta_i\right]\\
q_{s,i} &= \lim_{D\to\infty}\frac{1}{D} \E_\mathcal{P}\left[\bs{s}_i \cdot \bs{s}_i\right],\\
q_{w} &= \lim_{P\to\infty}\frac{1}{P} \E_\mathcal{P}\left[ \hat{\bs{w}} \cdot \hat{\bs{w}}\right],
\end{align*}
where $\bs{s}=\frac{1}{\sqrt{P}} F \hat{\bs{w}} \in \sR^{D}$ and $\bs s_i, \bs \beta_i \in \sR^{\phi_i D}$ denote the orthogonal projections of $\bs s$ and $\bs \beta$ onto subspace $i\in\{1,2\}$. 

The distribution $\mathcal{P}$ over which the expectations are taken is the joint distribution of all random quantities in the problem: the teacher weights $\bs \beta$, the random features $\bs F$ and the training data $\bs x$. 

The order parameters are one of the outputs of the replica computation deferred to SM~\ref{app:replica}. They are obtained by solving a set of non-linear equations (see Section \ref{app:saddle-point} of the SM).
The replica formalism allows also to obtain the asymptotic training error, in a similar fashion to~\citet{gerace2020generalisation}. In what follows, to gain more intuition, we focus on two simple cases.

\paragraph{Square loss regression}

We first consider the square loss regression setup $\ell (x,y) = (x-y)^2$ where $\hat f = f^0 = \text{id}$ and the labels are corrupted by additive noise, i.e. 
\begin{align}
    y_\mu = \frac{\bs \beta \cdot \bs x_\mu}{\sqrt D} + \eta_\mu, \quad \eta_\mu\sim\mathcal{N}(0, \Delta).
\end{align}
The expressions of the test and train error become very informative : 
\begin{align}
    \epsilon_g &= \frac{1}{2}\left(\rho + Q - 2 M \right),\\
    \epsilon_t &= \frac{\epsilon_g + \Delta/2}{(1+V)^2},
\end{align}
with
\begin{align*}
    V &= \kappa_1^2 \sum_i \sigx{i} v_{s,i} + \kappa_\star^2 v_w ,\\
    v_{s,i}&=\lim_{D\to\infty} \frac{1}{D} \sV_\mathcal{P} \left[\bs{s}_i \cdot \bs{s}_i\right], \\  
    v_{w}&=\lim_{P\to\infty} \frac{1}{P} \sV_\mathcal{P} \left[ \hat{\bs{w}} \cdot \hat{\bs{w}}\right] 
\end{align*}
where $\sV_\mathcal{P}$ denotes the variance over all random quantities in the problem. Similarly, the values of the order parameters $v_s, v_w$ are obtained by solving the set of equations given by the replica calculation.

Note here the surprisingly simple relation between the train loss and the test loss. One can invert this expression and write $\epsilon_g = \epsilon_t (1+V)^2 - \Delta/2$, showing that $V$ acts as a variance opening a generalization gap. 

\paragraph{Square loss classification}
Our framework is valid for any convex loss function, however the replica equations need to be evaluated numerically in the general case. For this reason, we focus here on the square loss classification setup\footnote{Note that for datasets with few classes, recent works~\cite{hui2020evaluation, demirkaya2020exploring} have shown that deep networks trained with MSE loss demonstrate comparable test-error performance to those trained with cross-entropy} i.e. $\ell (x,y) = (x-y)^2$ where $\hat f = f^0 = \text{sign}$, in which case the replica equations have a closed form which is both interpretable and easy to evaluate. In this case, the labels are corrupted by random label flipping of probability $\Delta$, i.e. 
\begin{align}
    y_\mu = \eta_\mu\ \text{sign}\left(\frac{\bs \beta \cdot \bs x_\mu}{\sqrt D}\right), \quad \eta_\mu = \begin{cases}
    1 \text{ w. prob. }1-\Delta\\
    -1 \text{ w. prob. }\Delta.
    \end{cases}
\end{align}
In this case, the expressions of the train and test error are:
\begin{align}
    \epsilon_g &= \frac{1}{\pi} \cos ^{-1}\left(\frac{M}{\sqrt{\rho Q}}\right),\\
    \epsilon_t &= \frac{1}{2(1+V)^2}\left( \rho + Q - 2 (1- 2 \Delta) M \right) \, .
\end{align}

% \begin{figure*}[!htb]
\begin{figure*}[h!]
    \centering
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=.49\linewidth]{figs-rf/agreement_parameter_wise_te_error_tanh_noise0.3_lamb0.001_regression.pdf}
    \includegraphics[width=.49\linewidth]{figs-rf/agreement_sample_wise_te_error_tanh_noise0.3_lamb0.001_regression.pdf}
    \caption{Regression}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}	   
    \includegraphics[width=.49\linewidth]{figs-rf/agreement_parameter_wise_te_error_tanh_noise0.3_lamb0.001_classification.pdf}
    \includegraphics[width=.49\linewidth]{figs-rf/agreement_sample_wise_te_error_tanh_noise0.3_lamb0.001_classification.pdf}
    \caption{Classification}
    \end{subfigure}
    \caption{\textbf{Anisotropic data strongly affects the double descent curves.} Theoretical results (solid curves) and numerical results (dots with vertical bars denoting standard deviation over 10 runs) agree even at moderate size $D=100$ for both regression (upper row) and classification (lower row) tasks.
    %Our analytical results allow us to extend far beyond the sizes achievable computationally. 
    We set $\sigma = \mathrm{Tanh}$, $\lambda=10^{-3}$ and $\Delta=0.3$. For the blue curve $r_x = r_\beta = 1$, for the orange curve $r_x = 10$ and $ r_\beta = 0.01$, 
    for the green
    % curve $r_x = 10$ and $ r_\beta = 1$ and for the red 
    curve $r_x = 10$ and $ r_\beta = 100$. In all cases $\phi_1 = 0.1$. \textit{Left:} parameter-wise profile at $N/D=1$. \textit{Right:} sample-wise profile at $P/D=1$.}
    \label{fig:agreement-noise}
\end{figure*}

\section{Effect of data structure on double descent}
\label{sec:results}

Before investigating the entire generalization phase space, we focus on ``slices" by either fixing the number of training samples $N$ and varying the number of parameters $P$ or conversely fixing $P$ and varying $N$. The main issue here is to investigate how the data structure affects the test error curves, and in particular the parameter-wise and sample-wise double descent phenomenon found for isotropic data.

We compare three cases. The first is the \emph{isotropic} setup where $r_x=1$ (blue curves in Fig.~\ref{fig:agreement-noise}). In the two next setups, the data is anisotropic with a small subspace ($\phi_1=0.1$) of large variance and a large subspace ($\phi_2=0.9$) of small variance. The ratio of the variances $r_x= \sigma_{x,1} / \sigma_{x,2}$ is set to 10, and their values are chosen to keep the total variance of the inputs unchanged: $\frac{1}{D}\E \Vert \bs x \Vert^2= \phi_1 \sigma_{x,1} + \phi_2 \sigma_{x,2}=1$.

We study two cases for the outputs: (i) the \emph{relevant salient features} scenario where the strong subspace is the most relevant ($r_\beta = \sigma_{\beta,1} / \sigma_{\beta,2} =100$, green curves in Fig.~\ref{fig:agreement-noise}); (ii) the \emph{irrelevant salient features} scenario, where the strong subspace has low relevance ($r_\beta=0.01$, orange curves in Fig.~\ref{fig:agreement-noise}), i.e. contributes very little to the output. In both cases, we choose the $\sigma_{\beta,i}$ such that the total variance of the outputs is unchanged: $\E y^2 = \phi_1 \sigma_{x,1} \sigma_{\beta,1} + \phi_2 \sigma_{x,2}\sigma_{\beta,2}=1$. 


\paragraph{Validity at finite size}
First we validate our main result by comparing our analytical predictions with the outcomes of numerical experiments, both for test loss (Fig.~\ref{fig:agreement-noise}) and the train loss (Fig.~\ref{fig:double-descent-training} of SM~\ref{app:train}). The agreement is already excellent for moderately large dimensions $D=100$, both in the parameter-wise curves and the sample-wise curves\footnote{In the classification setup, the variance of the numerical experiments is increased by the presence of label flipping.}. Note that the replica method, which relies on solving a set of scalar fixed point equations, is also computationally efficient. It allows here to probe ratios of $P/D$ and $N/D$ far beyond what is tractable by the numerics (P, D and N only appear in the replica equations through the values of the ratios $N/P$ and $P/D$). We also report the behavior of the order parameters $M, Q$ and $V$ in SM~\ref{app:saddle-point}. 

\paragraph{Relevant salient features}
When the salient features are relevant, the anisotropy of the data makes the task easier. This can be seen both in the parameter-wise profile: the test loss drops at $P = \phi_1 D$ (instead of $P=D$), and in the sample-wise profile: the test loss drops at $N = \phi_1 D$ (instead of $N = D$). These observations are in line with the results of~\citet{ghorbani2020neural} and show that relevant salient features make the problem low-dimensional with an effective dimension close to $\phi_1D$. The remaining features act as additional noise in the data. As explained in the former reference, this setup is the most akin to real-world tasks. For example, the most salient Fourier features of an image are often the most relevant to its recognition. In this sense, the impressive performance of kernel methods such as the Convolutional NTK on real-world datasets~\cite{arora2019harnessing} can be associated with the anisotropy of the data: feature learning is not required to beat the curse of dimensionality if the irrelevant features are weakly salient to begin with.

\vspace{-1em}

\paragraph{Irrelevant salient features} 
We focus next on the case where the salient features are weakly relevant (orange curve in Fig.~\ref{fig:agreement-noise}). In this case, these features carry very little signal and mainly act as a troublesome source of noise in input space. Hence, in the sample-wise curves, the test loss is always higher than the isotropic baseline (blue in Fig.~\ref{fig:agreement-noise}), showing the detrimental effect of these features. In the regression setup, we even observe a second peak appear, forming a sample-wise triple descent curve: the salient irrelevant subspace creates a ``linear peak"~\cite{d2020triple} at $N/D =\phi_1$, at which the system overfits the noise.

In the parameter-wise curves, an interesting crossover occurs: the irrelevant features are detrimental from small $P$, but become helpful at large $P$, as can be seen from the orange curve reaching a lower asymptotic value than the blue curve in the left panels of Fig.~\ref{fig:agreement-noise}. We associate this to the phenomenon discovered for linear regression in~\citet{richards2020asymptotics}, whereby adding noisy features acts as a form of implicit regularization. 
%In our setup, this regularization helps to fight the initialization variance~\cite{d2020double,adlam2020understanding} in the overparametrized regime.

\section{More data or more parameters?}
\label{sec:symmetry}

\begin{figure*}[htb]
    \centering
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-rf/phase_space_te_error_rx1_rb0.01_relu_noise0.0_lamb0.1_classification.pdf}
    \caption{Isotropic, noiseless}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-rf/phase_space_te_error_rx1_rb0.01_relu_noise0.3_lamb0.1_classification.pdf}
    \caption{Isotropic, $\Delta=0.4$}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-rf/phase_space_te_error_rx100_rb100.0_relu_noise0.0_lamb0.1_classification.pdf}
    \caption{Anisotropic, $\Delta=0$}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-rf/phase_space_te_error_rx100_rb100.0_relu_noise0.3_lamb0.1_classification.pdf}
    \caption{Anisoptropic, $\Delta=0.4$}
    \end{subfigure}
    \caption{\textbf{The symmetry of the generalization phase space vanishes when the data becomes noisy or anisotropic.} We studied the classification task for $\sigma = \mathrm{ReLU}$, $\lambda=0.1$. In the anisotropic phase spaces we set $\phi_1=0.01$, $r_x=100$, $r_\beta=100$.}
    \label{fig:phase-space-analytic}
\end{figure*}
% \vspace{-1pt}
\begin{figure*}[!ht]
\centering
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_MNIST_pca0_noise0.pdf}
    \caption{MNIST, noiseless}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_MNIST_pca0_noise0.5.pdf}
    \caption{MNIST, 50\% corruption}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_MNIST_pca1_noise0.pdf}
    \caption{MNIST PCA, noiseless}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_MNIST_pca1_noise0.5.pdf}
    \caption{MNIST PCA, 50\% corr.}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_CIFAR10_pca0_noise0.pdf}
    \caption{CIFAR10, noiseless}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_CIFAR10_pca0_noise0.5.pdf}
    \caption{CIFAR10, 50\% corruption}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_CIFAR10_pca1_noise0.pdf}
    \caption{CIFAR10 PCA}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}	   
    \includegraphics[width=\linewidth]{figs-nn/test_error_CIFAR10_pca1_noise0.5.pdf}
    \caption{CIFAR10 PCA, 50\% corr.}
    \end{subfigure}
    \caption{\textbf{Noisy labels and PCA transformation break the symmetry of the phase space.} \textit{Top:} MNIST, downsampled to $D=10\times 10$ images. \textit{Bottom:} CIFAR10, downsampled to $D=10\times 10$ images. In all cases, we represented the test error at convergence of 2-layer networks trained via gradient descent. The results are averaged over 10 runs.}
    \label{fig:phase-space}
\end{figure*}


In this section, we investigate both analytically and empirically 
how the structure of data shapes the generalization phase space. We first address this issue in the random feature model then confirm our findings in numerical experiments on real data.  

\subsection{Random feature model}

We display the test error of the random feature model in the $(N,P)$-phase space in Fig.~\ref{fig:phase-space-analytic}, focusing on the classification setting. In the noiseless isotropic setup, we see that the phase space is quasi-symmetric around the line $N=P$ (panel (a), Fig.~\ref{fig:phase-space-analytic}). We observe the usual overfitting peak of double descent along the interpolation threshold $N\sim P$ (dashed line, Fig.~\ref{fig:phase-space-analytic}).

\paragraph{Noisy labels} A clear asymmetry emerges when corrupting the labels (panel (b), Fig.~\ref{fig:phase-space-analytic}). In this case, the test error becomes higher everywhere, but particularly in two regions: the small-data region at $N\sim D$, marked by the vertical solid line, and near the interpolation threshold $N\sim P$, along the diagonal dashed line. In this setting, many data and few parameters becomes better in terms of generalization than many parameter-few data.

\paragraph{Structure of the inputs} When we make the input data anisotropic, in the relevant salient features setup, asymmetry emerges again (panel (c), Fig.~\ref{fig:phase-space-analytic}). In this case, the test error becomes lower everywhere: we saw already that the task becomes low-dimensional hence easier. However, despite the absence of noise in the labels, we see a vertical overfitting peak along $N\sim D$ (dashed line, Fig.~\ref{fig:phase-space-analytic}). As we discussed in the previous section, the non-salient features induce an effective noise in the data, which give rise to a ``triple descent" phase space, as was observed in~\cite{d2020triple} for the regression setup. Fig. \ref{fig:increasing-rx} of the SM shows how the disymmetry of the phase-space builds as we increase the anisotropy $r_x$ from 1, then vanishes when $r_x\to\infty$ as the non-salient features vanish, leaving an isotropic task of dimensionality $\phi_1$.

Finally, the asymmetry in the generalization phase space is strongest when the task is both noisy and anisotropic (panel (d), Fig.~\ref{fig:phase-space-analytic}). In this case, most of the overparametrized region $P>N$ is affected by overfitting: optimal performance is clearly achieved in the underparametrized region $P<N$.

\paragraph{Sources of variance}

The roles of $N$ and $P$ can be understood in terms of a bias-variance decomposition~\cite{d2020double,adlam2020understanding}. By overparametrizing, we average out the variance due to the randomness of the random features $\{\bs F_i\}_{i=1\ldots P}$, whereas by increasing the number of training examples we average out the variance due to (1) the randomness of the inputs $\{\bs x_\mu\}_{\mu=1\ldots N}$ and (2) the noise in the labels $\{\eta_\mu\}_{\mu=1\ldots N}$. 

In the isotropic noiseless setup, the random features and the input data follow the same distribution and the roles of $N$ and $P$ are symmetric since the random feature projection is given by $\sigma(\bs F_i \cdot \bs x_\mu/\sqrt D)$. However, in presence of corrupted labels or irrelevant inputs, increasing $N$ also averages out the extra sources of randomness in the data, and hence has a stronger effect on the test error than increasing $P$. 


\subsection{Neural networks}

We now turn to two-layer networks trained on MNIST and CIFAR10 to see if our analytical findings hold in a more realistic setting. To unify the dimensions and explore the $(N, P)$-phase space consistently, we downscale the images to $10\times 10$ pixels, such that $D=100$. We train using full-batch gradient descent for 3000 epochs, with a learning rate of 0.05 and momentum 0.9. The width $H$ of the hidden layer is varied from 4 to 512, and the number of examples $N$ in the dataset is varied from 256 to 32k. Note that in this case, $P = (D+1) H$ denotes the total number of parameters in both layers, therefore we only have access to the region $P>D$ of the landscape.

As can be seen in panels (a) and (e) of Fig.~\ref{fig:phase-space}, the test error phase space is almost symmetric around the interpolation threshold both for MNIST and CIFAR10, despite the vastly different magnitudes of the test error (down to 2\% for MNIST, against 54\% for CIFAR10). 
The double descent phenomenon is absent because of the training algorithm: gradient descent with finite-learning rate and momentum exerts an implicit regularization~\cite{gunasekar2017implicit}. Hence, the test error monotonically decays both as we increase $N$ and $P$. 
In order to confirm the role played by the data in shaping the generalization phase space we now study the effect of corrupting the labels and modifying the input distribution of the datasets.
%We then investigate how the properties of the dataset affect this symmetry following our conclusions on the random feature model.

\paragraph{Noisy labels}
We corrupt the data by shuffling 50\% of the labels of the training set, leaving the test set clean. This causes the lowest test error to rise to 46\% for MNIST and 76\% for CIFAR10. The effect on the corresponding phase spaces are shown in panels (b) and (f) of Fig.~\ref{fig:phase-space}. As observed analytically, the increase in test error is higher in the overparametrized region $P>N$ due to overfitting, which causes the phase space to appear less symmetric.

\paragraph{Structure of the inputs}
In order to make the data anisotropic, we apply a PCA transformation to the original datasets, then retain the top $D=100$ principal components as inputs. In this way, the first few features contain most of the relevant information, whereas the last features are essentially pure noise. Just like in the salient relevant features setup, generalization is improved by this preprocessing procedure: the minimum test error falls to 1\% for MNIST and 50\% on CIFAR10. Similarly to the case of noisy labels, we observe in panels (c) and (g) of Fig.~\ref{fig:phase-space} that the phase space becomes slightly less symmetric.

Finally, the asymmetry is strongest in the rightmost panels, where we applied the PCA transformation on top of corrupting the labels. As for the random features setup, the whole overparametrized region $P>N$ suffers from overfitting, particularly along the lines $N\sim P$ and near $N\sim D$. Again, having a lot of data is more valuable than having a lot of parameters.

% \paragraph{Summary}

% We have shown both analytically and empirically that the generalization phase space de-symmetrizes if (1) the labels are noisy or (2) the inputs are anisotropic : having more data (large $N$) becomes more valuable in these setups than having more parameters (large $P$). In the first case, the performance is deteriorated as the underlying classification rule is corrupted; having more training points allows to averaging over the noise. In the second case, performance is globally improved as the task becomes effectively lower dimensional. Nevertheless, irrelevant input dimensions become a source of noise which is more easily eliminated by increasing sample size than increasing model size.

\section{Conclusion}
Analytical explorations on isotropic data and empirical results on simple datasets tend to show that increasing model size is of same value as increasing sample size. However, this symmetry appears to be due to the ``clean" nature of the data considered and vanishes as soon as the inputs or the labels are noisy. We have shown that in such scenarios, increasing sample size becomes more valuable than increasing model size since it allows to average out the noise. These contrasting conclusions illustrate the need for a thorough analysis of the impact of data structure on learning, which may ultimately lead to more interpretable and explainable systems. Bridging the gap between what is theoretically tractable and what works in practice is a challenging task that will also motivate our future work. In the current paper, we investigated independent input variables. Future directions include the investigation of the structure of data with correlations within or across subspaces, and the study of representations of data. %before moving on to more complex settings. 

% \cite{ansuini2019intrinsic, chung2018classification, andrew2013deep}

==> dfdxcbxrhpmwxgqmtdsvvrxqthrzkvjb/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,bbm}

\def\ind{{\mathbbm{1}}}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}
\newcommand{\figleftt}{{\em Left}}
\newcommand{\figcentert}{{\em Center}}
\newcommand{\figrightt}{{\em Right}}
\newcommand{\figtopt}{{\em Top}}
\newcommand{\figbottomt}{{\em Bottom}}
\newcommand{\captionat}{{\em a}}
\newcommand{\captionbt}{{\em b}}
\newcommand{\captionct}{{\em c}}
\newcommand{\captiondt}{{\em d}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}

\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}
\def\rmtheta{{\mathbf{\Theta}}}
% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}


\DeclareMathOperator{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\vbar}[1]{\bigg\rvert_{#1}}
\newcommand\at[2]{\left.#1\right|_{#2}}
\newcommand{\bs}[1]{\boldsymbol{#1}}

\newcommand{\sigx}[1]{\sigma_{x,#1}}
\newcommand{\sigb}[1]{\sigma_{\beta,#1}}

\newcommand{\dd}{\mathrm{d}} %for integration
